Robust remote estimation over the collision channel in the presence of an intelligent jammer

We consider a sensor-receiver pair communicating over a wireless channel in the presence of a jammer who may launch a denial-of-service attack. We formulate a zero-sum game between a coordinator that jointly designs the transmission and estimation policies, and the jammer. We consider two cases depending on whether the jammer can sense the channel or not. We characterize a saddle-point equilibrium for the class of symmetric and unimodal probability density functions when the jammer cannot sense the channel. If the jammer can sense if the channel is being used, we provide an efficient algorithm that alternates between iterations of Projected Gradient Ascent and the Convex-Concave Procedure to find approximate First-order Nash-Equilibria. Our numerical results show that in certain cases the jammer may decide to launch a denial-of-service attack with the goal of deceiving the receiver even when the sensor decides not to transmit.

==> simulation.tex <==
%!TEX root = main.tex


In this section, we provide a numerical experiment to illustrate the performance of  \cref{eq:algorithm} under the random quantization scheme given in \cref{sec:increasing_quantizer}. Our simulation is similar to the ones in \cite{Doan:2018a}, however, we do not require any projection to a predefined compact set. As a result, the quantization intervals at each step in our algorithm are different and increasing in $k$.

We apply \cref{eq:algorithm} for solving the distributed variant of the popular linear regression problem. The goal of this problem is to find a linear relationship between a set of variables and some real valued outcome. That is, given a training set $S = \{(w_i,b_i)\in\mathbb{R}^{d}\times\mathbb{R}\}$ for $i=1,\cdots,n$. We want to find the solution of the following optimization problem
\begin{align}
\min_{x\in\mathbb{R}^{d}}\sum_{i=1}^n (w_i^Tx-b_i)^2,
\end{align}
%\begin{align*}
%\min_{x\in\mathbb{R}^{d}}\;\sum_{i=1}^n(w_i^Tx-b_i)^2.
%\end{align*}
In this case, we know that the optimal centralized solution can be efficiently found by solving a least squares problem. The challenge is to how to solve it efficiently in a decentralized fashion, under strict quantization constraints.

Suppose that $w_i\in\mathbb{R}^{5}$. We consider simulated training data sets where $(w_i,b_i)$, $i\in\{1,\cdots,n\}$, are generated randomly and independently according to the following uniform distributions: $w_i(j) \sim \mathcal{U}[0,0.65],  \ \ j\in\{1,\cdots,d\}$
and
$b_i \sim \mathcal{U}[0,0.45].$

We study the performance of our distributed gradient method on a undirected connected graph of $40$ nodes, i.e., $\mathcal{G}=(\mathcal{V},\mathcal{E})$ and $n = |\mathcal{V}|=40$. Our graph is generated randomly, similar to the ones in \cite{Doan:2018a}. Finally, the adjacency matrix $A$ is chosen as a Lazy Metropolis matrix corresponding to $\mathcal{G}$, i.e.,
\begin{align}
A = [a_{ij}] = \left\{\begin{array}{ll}
\big(2(\max\{|\mathcal{N}_i| , |\mathcal{N}_j|\}\big)^{-1}, & \text{ if } (i,j) \in \mathcal{E}\\
1-\sum_{j\in\mathcal{N}_i}a_{ij},& \text{ if } i = j \\
0, &\text{ otherwise. } %(i,j)\notin\mathcal{E} \text{ and } i\neq j\\
\end{array}\right.
\end{align}
%It is straightforward to verify that the Lazy Metropolis matrix $A$ is doubly stochastic. 

In this example, the state variables $x^i_k$ were quantized using $16$ bits.
%, without the need for periodic transmissions real numbers among agents.
In \cref{fig:my_label}, we clearly see the convergence of the quantized vs. the unquantized algorithm, which asymptotically achieve the same value of the objective function, but there is a slight degradation due to the quantization error. It is important to note that despite the fact that the instantaneous quantization error increases with time, our algorithm successfully compensates for that by driving the estimates swiftly to the desired optimal solution. Hence, the excellent asymptotic convergence.

%Finally, for the purpose of our simulation, we use the Matlab optimization toolbox to compute the optimal solutions, and use them as a reference to compare the performance of our algorithms.

\begin{comment}
    \begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{network.pdf}
    \caption{Network with 40 nodes and 123 communication links used in our distributed linear regression application.}
    \label{fig:graph_example}
\end{figure}
\end{comment}



\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{performance.pdf}
    \caption{Performance of our algorithm with (solid line) and without (dashed line) quantization. In this example, the state variables was quantized using 16 bits/dimension.}
    \label{fig:my_label}
\end{figure}

